End-to-end Learning for Short Text Expansion

Effectively making sense of short texts is a critical task for many real world applications such as search engines, social media services, and recommender systems. The task is particularly challenging as a short text contains very sparse information, often too sparse for a machine learning algorithm to pick up useful signals. A common practice for analyzing short text is to first expand it with external information, which is usually harvested from a large collection of longer texts. In literature, short text expansion has been done with all kinds of heuristics. We propose an end-to-end solution that automatically learns how to expand short text to optimize a given learning task. A novel deep memory network is proposed to automatically find relevant information from a collection of longer documents and reformulate the short text through a gating mechanism. Using short text classification as a demonstrating task, we show that the deep memory network significantly outperforms classical text expansion methods with comprehensive experiments on real world data sets.

==> tex/intro_old.tex <==
\section{Introduction}
Short texts ubiquitously appear as a means to succinctly convey information in everyday life. Such examples include microblogs, search queries, online questions, user comments, calendar items, and news titles. Accurately understanding short texts is an important task for many online applications, such as search engines, recommender systems, online social media, and conversational agents. Because of the succinctness and ambiguity of short texts, it is a challenging task for machines, and sometimes even for humans. 
Consider the scenarios where we come across a news feed titled ``\emph{Sequestration in Fiscal 2016}''; in literature survey, we encounter a paper called ``\emph{Recognizing groceries {in situ} using {in vitro} training data}''; in online social media, someone posted a status: ``\emph{Watching that movie makes me ROFL!}''. The meaning of these short texts may not be obvious at the first sight. What will the human do?

% brief description of how humans solve it 
With the prevalence of search engines, a spontaneous response of human users is to query the short text in a search engine and look at returned results. The searcher expects the results contain rich and elaborate information about the short text in the forms of definitions, paraphrases, examples, synonyms, related concepts, and even illustrations such as images and videos. The search engine may inevitably return noisy and irrelevant results, but the searcher knows where to pay her attention and glean just the information she wants. To achieve a thorough understanding, human searchers often update their queries and search for multiple iterations.

The Web users leverage the Web pages to understand the short texts (queries). Therefore, in this paper, we study short text expansion with external long documents.

In literature, leveraging the vast volume of external data 
and online information is proven to be an effective strategy for short text understanding tasks.

It is adopted in query expansion \cite{buckley1995automatic}, short text classification \cite{sahami2006web, phan2008learning}, semantic relatedness analysis \cite{gabrilovich2007computing}, question answering \cite{dumais2002web}. However, the information retrieval step in previous works is one of many stages in the entire machine learning pipeline, whose errors may be propagated onto later stages. When the external data source is noisy, the accumulated errors may not benefit or even harm the performance of downstream machine learning tasks.

% this inspires algorithms that leverages web search to enhance short text representation, overcoming sparseness. However, many of them are heuristics and not aware of the downstream machine learning tasks that uses these representations.

% this strategy inspires machine learning algorithms too. Indeed, many algorithms leverage the vast amount of online information to enrich the representation of short text in question and achieve better performance in data mining tasks.
% What's missing in this strategy is the mechanisms of humans attention and iterative search is guided by a learning goal.



\begin{comment}
% Short text is a ubiquitous phenomenon that appears wherever information is expressed succinctly or entered in a short time. Examples include microblogs, search queries, online questions, user comments, calendar items, and news titles. Accurately classifying short texts into semantic categories is an important task for many applications, such as search engines, recommender systems, online social media, and conversational agents. Though it takes little effort for humans to understand a piece of text with only a few words, it is a challenging task for machines because of the sparse and ambiguous nature of short text.



Two main approaches exist for handling short text classification.
The first approach is to exploit word similarity and represent short text using latent dimensions rather than the naive `bag of words'. The latent dimensions can be predefined concepts \cite{bag_of_concepts}, probabilistic topics \cite{universal_topic_model}, or learned embeddings \cite{LINE, PTE}. By representing semantically related words close to each other, the new representation effectively reduces the dimensionality of  `bag-of-words' approach and alleviates data sparsity. However, for extremely short texts, this approach can still suffer from lack of enough information \cite{TKTK}.

The second approach is to exploit document similarity and enrich a piece of short text with other semantically related documents. These documents are usually retrieved efficiently from a large, indexed document collection, such as the Web \cite{web_kernel}. This approach is closely related to pseudo-relevance feedback in information retrieval \cite{PRF}, where the initial search query is refined by relevant documents it retrieves. In general, one can perform multiple rounds of retrieval and query refinement \cite{iterative_feedback}. However, it is difficult to determine the importance weights for retrieved documents in query refinement. As a result, this approach often introduces the risk of concept drift \cite{PRF_concept_drift}.

\end{comment}
We aim at designing a machine learning algorithm that emulates the human's search skills. It not only knows to tap into massive external data using search interface, but also \emph{learns} how to search effectively to perform well in a downstream machine learning task. Instead of paying equal attention to all returned results, the algorithm should learn to pay more attention to relevant results and less to irrelevant ones. It should also avoid being led astray by the returned results if none of them are relevant enough. To carry new information to the downstream task or use it in more search iterations, the algorithm need to maintain and update an internal representation of the short text. Furthermore, all these steps are trained in an end-to-end fashion, with the ultimate goal of achieving good performance in a downstream learning task.

To implement this idea, we propose a new algorithm based on memory networks. The network holds search results in its memory, which is relatively large to ensure a high recall of potentially relevant results. In the face of noisy or irrelevant results, it employs the attention mechanism to put proper weights on relevant and non-relevant results. Furthermore, it uses a gating mechanism to determine which information to retain and which to discard towards the goal of learning.  The iterative search process of a human searcher is naturally encoded in a recurrent network structure. For the final machine learning task, we use short text classification as it is an important and popular task.
{\color{red} Hard attention? }

% We aim at designing a machine learning algorithm that emulates the human's search strategy and create short text representations directly towards the goal of a machine learning task. We use short text classi. Given a short text, the algorithm leverages the vast and easily accessible online information, and learn the short text representation in an end-to-end approach. In the face of noisy and irrelevant search results, it learns to pay proper attention to those results relevant to the goal of learning. It can refine the query and perform multiple rounds of search. Furthermore, all these steps are \emph{learned}  training data, so the algorithm can be easily adapted across different domains of short text classification tasks.

% These design goals are realized using a deep memory network with attention mechanism. The network learns low-dimensional text embedding for both short texts and retrieved results. It holds retrieved results in memory and uses the attention mechanism to determine the importance of each result. The results are used to augment the short text in question. Finally, the iterative search process of a human searcher is naturally encoded in a recurrent network structure.


In this paper, we design such an automate process with a deep memory network. The network simulates the process of Web user searching on the search engines, and is trained in an end-to-end fashion. 
Given a short text, it first retrieve a set of potentially relevant documents to the short text from the entire collections, which may be noisy. Therefore, attention mechanisms~\cite{} are used to determine which documents should be paid attention to. Both the soft and hard attention mechanisms are used, which either defines a probability distribution over the documents or focuses on an individual document. With the attention mechanism, some new information from the long documents can be identified. It is natural to reformulate the short text by integrating information from the original feature and the information attended from the long documents. In classical methods of query expansion, this is achieved by a linear combination of the two information, and a scalar coefficient is empirically chosen for the combination, which is very heuristic. In our network, a principled solution the Gated Recurrent Unit (GRU)~\cite{} to combine the two sources of information, in which the weights are automatically determined. As a Web user, the search can continue multiple runs by reformulating the query. Therefore, our deep memory network also allows to expand the short text multiple times by treating the reformulated short text as initial inputs. The final representation of short text is used for prediction. In this paper, we take the task of short text classification as an example. Based on the classification objective, the whole network is trained by backpropagation.

We evaluate our algorithm on short text data sets of different genres, including Wikipedia article titles (general domain), computer science publication titles (scientific domain), and sentiment classification of tweets (social media). Experimental results show that our proposed deep memory network significantly outperforms classical heuristic query expansion methods and methods only using short text features.

To summarize, we make the following contributions:
\begin{itemize}
	\item We propose a novel end-to-end solution for short text expansion with long documents. A variant of deep memory network is proposed to attend relevant information from the relevant documents and integrate the attended information with the original information. 
    \item We conduct extensive experiments on real-world short text data sets. Experimental results on short text classification show that our proposed deep memory networks significantly outperforms the traditional query expansion methods and the methods which only use the features in short text.
   \end{itemize}

\noindent \textbf{Organizations.} The rest of this paper is organized as follows. Section 2 discusses the related work. Section 3 formally defined the problem of short text expansion followed by our end-to-end solution in Section 4. Section 5 report the experimental results, and we conclude this paper in Section 6. 

\begin{comment}
The logic:

(1) Short text are ubiquitous, an important problem, but challenging because of feature sparseness and ambiguity

(2) In practice, what a search engine user would to input a search query, fine tune the query based on the search results, iteratively doing this until ... Can we design an algorithm to simulate this base?

(3) In this paper, we design such an algorithm based on deep memory networks ..., 

two scenarios: (a) long documents are available (b) only short documents are available ...

To summarize, in this paper, we make the following contributions:

\begin{itemize}
	\item We propose to study short text classification with long documents ...
    \item We propose a type of memory network (??)
    \item Experimental results ...
\end{itemize}


\end{comment}








==> tex/problem_definition.tex <==
\section{Problem Definition}
Short texts appear in a variety of applications such as user queries in search engines and user-generated content in social media. Understanding the meaning of short texts is critical for these applications. However, the problem is very challenging since the short texts contain only a few words, the information of which are very sparse and ambiguous. We first formally define short text as follows:

\begin{definition}
	\label{def::short-text}
	\textbf{(Short text.)}
	\textsl{A piece of \emph{short text} $w$ is represented as a sequence of words $w=(w_1,w_2,\ldots, w_n)$, where $n$ is usually very small (e.g., less than 10).}  
\end{definition}

To understand a piece of short text, a common practice of a Web user is formulating the short text as a search query, and then understand the short text by leveraging the relevant Web pages returned by the search engines. In other words, the Web user is leveraging the hug collection of Web pages for short text understanding. Therefore, in this paper, we study how to leverage external documents for expanding the representations of short texts and understanding the meanings of short texts. Many corpus are available for short text expansion and expansion, e.g., the entire Wikipedia articles and scientific literatures. We define external long documents as follows:

\begin{definition}
	\label{def::external-documents}
	\textbf{(External Long Documents.) }
	\textsl{A collection of \emph{long documents} is denoted as $\calC =\{d_i\}$, where $d_i$ is a long document and is also represented as a sequence of words.}
\end{definition}


However, given a short text $q$ and a large collection of long documents $\calC$, how can we find the relevant documents to expand the short text? In this paper, we aim to design an automate process. Of course, such an automate process requires supervision. We take the task of short text classification as an example to provide the supervision. Formally, our problem can be formulated as follows:

\begin{definition}
	\label{def::problem_definition}
	\textbf{(Problem Definition.)}
	\textsl{Given a collection of long documents $\calC$, we aim to learn a function than expands a short text $q$ into a richer representation $q'$, i.e., $q'=f(q, \calC)$. Based on the richer representation $q'$, we can accurately classify the short text into one of predefined categories $\calY$.
}
\end{definition}

In the next section, we introduce an end-to-end solution based on deep memory networks. 
